Trainable Highly-expressive Activation Functions

Nonlinear activation functions are pivotal to the success of deep neural nets, and choosing the appropriate activation function can significantly affect their performance. Most networks use fixed activation functions (e.g., ReLU, GELU, etc.), and this choice might limit their expressiveness. Furthermore, different layers may benefit from diverse activation functions. Consequently, there has been a growing interest in trainable activation functions. In this paper, we introduce DiTAC, a trainable highly-expressive activation function based on an efficient diffeomorphic transformation (called CPAB). Despite introducing only a negligible number of trainable parameters, DiTAC enhances model expressiveness and performance, often yielding substantial improvements. It also outperforms existing activation functions (regardless whether the latter are fixed or trainable) in tasks such as semantic segmentation, image generation, regression problems, and image classification. Our code is available at https://github.com/BGU-CS-VIL/DiTAC.

==> figures/raw/cpab_act_for_method/epoch_0_fig_b.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{190,190,190}
\definecolor{lightblue}{RGB}{173,216,230}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle x\)},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
y label style={at={(axis description cs:-0.12,.5)},anchor=south},
xmin=-4.90925598144531, xmax=5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Density of \(\displaystyle x\)},
ymin=0, ymax=164059.35,
ytick style={color=black},
%
grid=both,
grid style={line width=.1pt, draw=gray!10},
major grid style={line width=.2pt,draw=gray!20},
minor x tick num=1,
minor y tick num=1,
%
]
\draw[draw=black,fill=lightblue] (axis cs:-5,0) rectangle (axis cs:-4.5,4);
\draw[draw=black,fill=lightblue] (axis cs:-4.5,0) rectangle (axis cs:-4,5);
\draw[draw=black,fill=lightblue] (axis cs:-4,0) rectangle (axis cs:-3.5,5);
\draw[draw=black,fill=lightblue] (axis cs:-3.5,0) rectangle (axis cs:-3,15);
\draw[draw=black,fill=lightblue] (axis cs:-3,0) rectangle (axis cs:-2.5,74);
\draw[draw=black,fill=lightblue] (axis cs:-2.5,0) rectangle (axis cs:-2,341);
\draw[draw=black,fill=lightblue] (axis cs:-2,0) rectangle (axis cs:-1.5,1798);
\draw[draw=black,fill=lightblue] (axis cs:-1.5,0) rectangle (axis cs:-1,8434);
\draw[draw=black,fill=lightblue] (axis cs:-1,0) rectangle (axis cs:-0.5,32955);
\draw[draw=black,fill=lightblue] (axis cs:-0.5,0) rectangle (axis cs:0,88770);
\draw[draw=black,fill=lightblue] (axis cs:0,0) rectangle (axis cs:0.5,153942);
\draw[draw=black,fill=lightblue] (axis cs:0.5,0) rectangle (axis cs:1,156247);
\draw[draw=black,fill=lightblue] (axis cs:1,0) rectangle (axis cs:1.5,147650);
\draw[draw=black,fill=lightblue] (axis cs:1.5,0) rectangle (axis cs:2,143272);
\draw[draw=black,fill=lightblue] (axis cs:2,0) rectangle (axis cs:2.5,115634);
\draw[draw=black,fill=lightblue] (axis cs:2.5,0) rectangle (axis cs:3,79614);
\draw[draw=black,fill=lightblue] (axis cs:3,0) rectangle (axis cs:3.5,42760);
\draw[draw=black,fill=lightblue] (axis cs:3.5,0) rectangle (axis cs:4,18629);
\draw[draw=black,fill=lightblue] (axis cs:4,0) rectangle (axis cs:4.5,6604);
\draw[draw=black,fill=lightblue] (axis cs:4.5,0) rectangle (axis cs:5,2502);
\end{axis}

\end{tikzpicture}


==> figures/raw/learned_functions_pspnet/epoch0/ditac_with_gelu_epoch_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{dodgerblue}{RGB}{30,144,255}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle x\)},
xmin=-4, xmax=4,
xtick style={color=black},
y grid style={darkgray176},
% ylabel style={rotate=-90.0},
ylabel={\(\displaystyle v^{\theta}(x)\)},
ymin=-2, ymax=4,
ytick style={color=black},
y label style={at={(axis description cs:-0.08,.5)},anchor=south},
x label style={at={(axis description cs:.5,-0.15)}},
]
\addplot [semithick, dodgerblue]
table {%
-4 -0.00012671947479248
-3.91919183731079 -0.00017415032198187
-3.83838391304016 -0.000237708140048198
-3.75757575035095 -0.000322291336487979
-3.67676758766174 -0.000434250541729853
-3.59595966339111 -0.000581064610742033
-3.5151515007019 -0.000772497849538922
-3.4343433380127 -0.00102003407664597
-3.35353541374207 -0.00133783894125372
-3.27272725105286 -0.00174294819589704
-3.19191908836365 -0.00225554686039686
-3.11111116409302 -0.00289930240251124
-3.03030300140381 -0.00370162911713123
-2.9494948387146 -0.00469404365867376
-2.86868691444397 -0.0059120487421751
-2.78787875175476 -0.00739550217986107
-2.70707082748413 -0.00918773841112852
-2.62626266479492 -0.011336050927639
-2.54545450210571 -0.0138899739831686
-2.46464657783508 -0.0169011298567057
-2.38383841514587 -0.0204212907701731
-2.30303025245667 -0.0245009362697601
-2.22222232818604 -0.0291870050132275
-2.14141416549683 -0.0345202684402466
-2.06060600280762 -0.0405327528715134
-1.9797979593277 -0.047244131565094
-1.89898991584778 -0.0546584464609623
-1.81818187236786 -0.0627603307366371
-1.73737370967865 -0.0715113654732704
-1.65656566619873 -0.0808464661240578
-1.57575762271881 -0.0906704068183899
-1.4949494600296 -0.100854992866516
-1.41414141654968 -0.11123663187027
-1.33333337306976 -0.121614933013916
-1.25252521038055 -0.131752207875252
-1.17171716690063 -0.141373917460442
-1.09090912342072 -0.150170683860779
-1.01010096073151 -0.157801449298859
-0.929292917251587 -0.163898140192032
-0.848484873771667 -0.168071269989014
-0.767676770687103 -0.169917285442352
-0.686868667602539 -0.169026538729668
-0.60606062412262 -0.164992272853851
-0.525252521038055 -0.157420203089714
-0.444444447755814 -0.136135429143906
-0.363636374473572 -0.102917484939098
-0.282828271389008 -0.0652408301830292
-0.202020198106766 -0.0264270659536123
-0.121212124824524 0.0186216402798891
-0.0404040440917015 0.0726511403918266
0.0404040440917015 0.136192142963409
0.121212124824524 0.208004966378212
0.202020198106766 0.285563558340073
0.282828271389008 0.367011308670044
0.363636374473572 0.449168980121613
0.444444447755814 0.532091796398163
0.525252521038055 0.617169499397278
0.60606062412262 0.708203434944153
0.686868667602539 0.8033567070961
0.767676770687103 0.901383101940155
0.848484873771667 1.00022900104523
0.929292917251587 1.09612119197845
1.01010096073151 1.18603146076202
1.09090912342072 1.27200186252594
1.17171716690063 1.35221946239471
1.25252521038055 1.42534720897675
1.33333337306976 1.49322760105133
1.41414141654968 1.55731081962585
1.4949494600296 1.61737036705017
1.57575762271881 1.67510509490967
1.65656566619873 1.73091506958008
1.73737370967865 1.78542459011078
1.81818187236786 1.83867359161377
1.89898991584778 1.89071893692017
1.9797979593277 1.94162786006927
2.06060600280762 2.0200731754303
2.14141416549683 2.10689377784729
2.22222232818604 2.193035364151
2.30303025245667 2.27852916717529
2.38383841514587 2.36341714859009
2.46464657783508 2.44774556159973
2.54545450210571 2.53156447410583
2.62626266479492 2.61492657661438
2.70707082748413 2.69788289070129
2.78787875175476 2.78048324584961
2.86868691444397 2.86277484893799
2.9494948387146 2.94480085372925
3.03030300140381 3.02660131454468
3.11111116409302 3.10821175575256
3.19191908836365 3.18966341018677
3.27272725105286 3.27098441123962
3.35353541374207 3.35219764709473
3.4343433380127 3.4333233833313
3.5151515007019 3.51437902450562
3.59595966339111 3.59537863731384
3.67676758766174 3.67633318901062
3.75757575035095 3.75725340843201
3.83838391304016 3.8381462097168
3.91919183731079 3.91901755332947
4 3.99987316131592
};
\addplot [semithick, black, dashed]
table {%
-4 -0.00012671947479248
-3.91919183731079 -0.00017415032198187
-3.83838391304016 -0.000237708140048198
-3.75757575035095 -0.000322291336487979
-3.67676758766174 -0.000434250541729853
-3.59595966339111 -0.000581064610742033
-3.5151515007019 -0.000772497849538922
-3.4343433380127 -0.00102003407664597
-3.35353541374207 -0.00133783894125372
-3.27272725105286 -0.00174294819589704
-3.19191908836365 -0.00225554686039686
-3.11111116409302 -0.00289930240251124
-3.03030300140381 -0.00370162911713123
-2.9494948387146 -0.00469404365867376
-2.86868691444397 -0.0059120487421751
-2.78787875175476 -0.00739550217986107
-2.70707082748413 -0.00918773841112852
-2.62626266479492 -0.011336050927639
-2.54545450210571 -0.0138899739831686
-2.46464657783508 -0.0169011298567057
-2.38383841514587 -0.0204212907701731
-2.30303025245667 -0.0245009362697601
-2.22222232818604 -0.0291870050132275
-2.14141416549683 -0.0345202684402466
-2.06060600280762 -0.0405327528715134
-1.9797979593277 -0.047244131565094
-1.89898991584778 -0.0546584464609623
-1.81818187236786 -0.0627603307366371
-1.73737370967865 -0.0715113654732704
-1.65656566619873 -0.0808464661240578
-1.57575762271881 -0.0906704068183899
-1.4949494600296 -0.100854992866516
-1.41414141654968 -0.11123663187027
-1.33333337306976 -0.121614933013916
-1.25252521038055 -0.131752207875252
-1.17171716690063 -0.141373917460442
-1.09090912342072 -0.150170683860779
-1.01010096073151 -0.157801449298859
-0.929292917251587 -0.163898140192032
-0.848484873771667 -0.168071269989014
-0.767676770687103 -0.169917285442352
-0.686868667602539 -0.169026538729668
-0.60606062412262 -0.164992272853851
-0.525252521038055 -0.157420203089714
-0.444444447755814 -0.145938068628311
-0.363636374473572 -0.130205377936363
-0.282828271389008 -0.109922401607037
-0.202020198106766 -0.084838479757309
-0.121212124824524 -0.0547589734196663
-0.0404040440917015 -0.0195509307086468
0.0404040440917015 0.0208531115204096
0.121212124824524 0.0664531588554382
0.202020198106766 0.117181718349457
0.282828271389008 0.17290586233139
0.363636374473572 0.233430996537209
0.444444447755814 0.298506379127502
0.525252521038055 0.367832332849503
0.60606062412262 0.441068351268768
0.686868667602539 0.51784211397171
0.767676770687103 0.597759485244751
0.848484873771667 0.680413603782654
0.929292917251587 0.765394747257233
1.01010096073151 0.852299511432648
1.09090912342072 0.940738439559937
1.17171716690063 1.03034329414368
1.25252521038055 1.12077295780182
1.33333337306976 1.21171844005585
1.41414141654968 1.30290472507477
1.4949494600296 1.39409446716309
1.57575762271881 1.48508715629578
1.65656566619873 1.57571911811829
1.73737370967865 1.66586244106293
1.81818187236786 1.75542151927948
1.89898991584778 1.84433150291443
1.9797979593277 1.93255388736725
2.06060600280762 2.0200731754303
2.14141416549683 2.10689377784729
2.22222232818604 2.193035364151
2.30303025245667 2.27852916717529
2.38383841514587 2.36341714859009
2.46464657783508 2.44774556159973
2.54545450210571 2.53156447410583
2.62626266479492 2.61492657661438
2.70707082748413 2.69788289070129
2.78787875175476 2.78048324584961
2.86868691444397 2.86277484893799
2.9494948387146 2.94480085372925
3.03030300140381 3.02660131454468
3.11111116409302 3.10821175575256
3.19191908836365 3.18966341018677
3.27272725105286 3.27098441123962
3.35353541374207 3.35219764709473
3.4343433380127 3.4333233833313
3.5151515007019 3.51437902450562
3.59595966339111 3.59537863731384
3.67676758766174 3.67633318901062
3.75757575035095 3.75725340843201
3.83838391304016 3.8381462097168
3.91919183731079 3.91901755332947
4 3.99987316131592
};
\end{axis}

\end{tikzpicture}


==> figures/raw/learned_functions_pspnet/epoch0/ditac_with_relu_epoch_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{dodgerblue}{RGB}{30,144,255}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle x\)},
xmin=-4, xmax=4,
xtick style={color=black},
y grid style={darkgray176},
% ylabel style={rotate=-90.0},
ylabel={\(\displaystyle v^{\theta}(x)\)},
ymin=-2, ymax=4,
ytick style={color=black},
y label style={at={(axis description cs:-0.2,.5)},anchor=south},
x label style={at={(axis description cs:.5,-0.15)}},
]
\addplot [semithick, dodgerblue]
table {%
-4 -0.00012671947479248
-3.91919183731079 -0.00017415032198187
-3.83838391304016 -0.000237708140048198
-3.75757575035095 -0.000322291336487979
-3.67676758766174 -0.000434250541729853
-3.59595966339111 -0.000581064610742033
-3.5151515007019 -0.000772497849538922
-3.4343433380127 -0.00102003407664597
-3.35353541374207 -0.00133783894125372
-3.27272725105286 -0.00174294819589704
-3.19191908836365 -0.00225554686039686
-3.11111116409302 -0.00289930240251124
-3.03030300140381 -0.00370162911713123
-2.9494948387146 -0.00469404365867376
-2.86868691444397 -0.0059120487421751
-2.78787875175476 -0.00739550217986107
-2.70707082748413 -0.00918773841112852
-2.62626266479492 -0.011336050927639
-2.54545450210571 -0.0138899739831686
-2.46464657783508 -0.0169011298567057
-2.38383841514587 -0.0204212907701731
-2.30303025245667 -0.0245009362697601
-2.22222232818604 -0.0291870050132275
-2.14141416549683 -0.0345202684402466
-2.06060600280762 -0.0405327528715134
-1.9797979593277 -0.047244131565094
-1.89898991584778 -0.0546584464609623
-1.81818187236786 -0.0627603307366371
-1.73737370967865 -0.0715113654732704
-1.65656566619873 -0.0808464661240578
-1.57575762271881 -0.0906704068183899
-1.4949494600296 -0.100854992866516
-1.41414141654968 -0.11123663187027
-1.33333337306976 -0.121614933013916
-1.25252521038055 -0.131752207875252
-1.17171716690063 -0.141373917460442
-1.09090912342072 -0.150170683860779
-1.01010096073151 -0.157801449298859
-0.929292917251587 -0.163898140192032
-0.848484873771667 -0.168071269989014
-0.767676770687103 -0.169917285442352
-0.686868667602539 -0.169026538729668
-0.60606062412262 -0.164992272853851
-0.525252521038055 -0.157420203089714
-0.444444447755814 -0.136135429143906
-0.363636374473572 -0.102917484939098
-0.282828271389008 -0.0652408301830292
-0.202020198106766 -0.0264270659536123
-0.121212124824524 0.0186216402798891
-0.0404040440917015 0.0726511403918266
0.0404040440917015 0.136192142963409
0.121212124824524 0.208004966378212
0.202020198106766 0.285563558340073
0.282828271389008 0.367011308670044
0.363636374473572 0.449168980121613
0.444444447755814 0.532091796398163
0.525252521038055 0.617169499397278
0.60606062412262 0.708203434944153
0.686868667602539 0.8033567070961
0.767676770687103 0.901383101940155
0.848484873771667 1.00022900104523
0.929292917251587 1.09612119197845
1.01010096073151 1.18603146076202
1.09090912342072 1.27200186252594
1.17171716690063 1.35221946239471
1.25252521038055 1.42534720897675
1.33333337306976 1.49322760105133
1.41414141654968 1.55731081962585
1.4949494600296 1.61737036705017
1.57575762271881 1.67510509490967
1.65656566619873 1.73091506958008
1.73737370967865 1.78542459011078
1.81818187236786 1.83867359161377
1.89898991584778 1.89071893692017
1.9797979593277 1.94162786006927
2.06060600280762 2.0200731754303
2.14141416549683 2.10689377784729
2.22222232818604 2.193035364151
2.30303025245667 2.27852916717529
2.38383841514587 2.36341714859009
2.46464657783508 2.44774556159973
2.54545450210571 2.53156447410583
2.62626266479492 2.61492657661438
2.70707082748413 2.69788289070129
2.78787875175476 2.78048324584961
2.86868691444397 2.86277484893799
2.9494948387146 2.94480085372925
3.03030300140381 3.02660131454468
3.11111116409302 3.10821175575256
3.19191908836365 3.18966341018677
3.27272725105286 3.27098441123962
3.35353541374207 3.35219764709473
3.4343433380127 3.4333233833313
3.5151515007019 3.51437902450562
3.59595966339111 3.59537863731384
3.67676758766174 3.67633318901062
3.75757575035095 3.75725340843201
3.83838391304016 3.8381462097168
3.91919183731079 3.91901755332947
4 3.99987316131592
};
\addplot [semithick, black, dashed]
table {%
-4 0
-3.91919183731079 0
-3.83838391304016 0
-3.75757575035095 0
-3.67676758766174 0
-3.59595966339111 0
-3.5151515007019 0
-3.4343433380127 0
-3.35353541374207 0
-3.27272725105286 0
-3.19191908836365 0
-3.11111116409302 0
-3.03030300140381 0
-2.9494948387146 0
-2.86868691444397 0
-2.78787875175476 0
-2.70707082748413 0
-2.62626266479492 0
-2.54545450210571 0
-2.46464657783508 0
-2.38383841514587 0
-2.30303025245667 0
-2.22222232818604 0
-2.14141416549683 0
-2.06060600280762 0
-1.9797979593277 0
-1.89898991584778 0
-1.81818187236786 0
-1.73737370967865 0
-1.65656566619873 0
-1.57575762271881 0
-1.4949494600296 0
-1.41414141654968 0
-1.33333337306976 0
-1.25252521038055 0
-1.17171716690063 0
-1.09090912342072 0
-1.01010096073151 0
-0.929292917251587 0
-0.848484873771667 0
-0.767676770687103 0
-0.686868667602539 0
-0.60606062412262 0
-0.525252521038055 0
-0.444444447755814 0
-0.363636374473572 0
-0.282828271389008 0
-0.202020198106766 0
-0.121212124824524 0
-0.0404040440917015 0
0.0404040440917015 0.0404040440917015
0.121212124824524 0.121212124824524
0.202020198106766 0.202020198106766
0.282828271389008 0.282828271389008
0.363636374473572 0.363636374473572
0.444444447755814 0.444444447755814
0.525252521038055 0.525252521038055
0.60606062412262 0.60606062412262
0.686868667602539 0.686868667602539
0.767676770687103 0.767676770687103
0.848484873771667 0.848484873771667
0.929292917251587 0.929292917251587
1.01010096073151 1.01010096073151
1.09090912342072 1.09090912342072
1.17171716690063 1.17171716690063
1.25252521038055 1.25252521038055
1.33333337306976 1.33333337306976
1.41414141654968 1.41414141654968
1.4949494600296 1.4949494600296
1.57575762271881 1.57575762271881
1.65656566619873 1.65656566619873
1.73737370967865 1.73737370967865
1.81818187236786 1.81818187236786
1.89898991584778 1.89898991584778
1.9797979593277 1.9797979593277
2.06060600280762 2.06060600280762
2.14141416549683 2.14141416549683
2.22222232818604 2.22222232818604
2.30303025245667 2.30303025245667
2.38383841514587 2.38383841514587
2.46464657783508 2.46464657783508
2.54545450210571 2.54545450210571
2.62626266479492 2.62626266479492
2.70707082748413 2.70707082748413
2.78787875175476 2.78787875175476
2.86868691444397 2.86868691444397
2.9494948387146 2.9494948387146
3.03030300140381 3.03030300140381
3.11111116409302 3.11111116409302
3.19191908836365 3.19191908836365
3.27272725105286 3.27272725105286
3.35353541374207 3.35353541374207
3.4343433380127 3.4343433380127
3.5151515007019 3.5151515007019
3.59595966339111 3.59595966339111
3.67676758766174 3.67676758766174
3.75757575035095 3.75757575035095
3.83838391304016 3.83838391304016
3.91919183731079 3.91919183731079
4 4
};
\end{axis}

\end{tikzpicture}


==> figures/raw/learned_functions_pspnet/epoch0/vf_epoch_0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate}{RGB}{210,105,30}
\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle x\)},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel style={rotate=-90.0},
ylabel={\(\displaystyle v(x)\)},
ymin=-0.00818644985556602, ymax=0.171915446966887,
ytick style={color=black}
]
\addplot [semithick, black, dashed]
table {%
0 0
0.0101010101010101 0
0.0202020202020202 0
0.0303030303030303 0
0.0404040404040404 0
0.0505050505050505 0
0.0606060606060606 0
0.0707070707070707 0
0.0808080808080808 0
0.0909090909090909 0
0.101010101010101 0
0.111111111111111 0
0.121212121212121 0
0.131313131313131 0
0.141414141414141 0
0.151515151515152 0
0.161616161616162 0
0.171717171717172 0
0.181818181818182 0
0.191919191919192 0
0.202020202020202 0
0.212121212121212 0
0.222222222222222 0
0.232323232323232 0
0.242424242424242 0
0.252525252525253 0
0.262626262626263 0
0.272727272727273 0
0.282828282828283 0
0.292929292929293 0
0.303030303030303 0
0.313131313131313 0
0.323232323232323 0
0.333333333333333 0
0.343434343434343 0
0.353535353535354 0
0.363636363636364 0
0.373737373737374 0
0.383838383838384 0
0.393939393939394 0
0.404040404040404 0
0.414141414141414 0
0.424242424242424 0
0.434343434343434 0
0.444444444444444 0
0.454545454545455 0
0.464646464646465 0
0.474747474747475 0
0.484848484848485 0
0.494949494949495 0
0.505050505050505 0
0.515151515151515 0
0.525252525252525 0
0.535353535353535 0
0.545454545454546 0
0.555555555555556 0
0.565656565656566 0
0.575757575757576 0
0.585858585858586 0
0.595959595959596 0
0.606060606060606 0
0.616161616161616 0
0.626262626262626 0
0.636363636363636 0
0.646464646464647 0
0.656565656565657 0
0.666666666666667 0
0.676767676767677 0
0.686868686868687 0
0.696969696969697 0
0.707070707070707 0
0.717171717171717 0
0.727272727272727 0
0.737373737373737 0
0.747474747474748 0
0.757575757575758 0
0.767676767676768 0
0.777777777777778 0
0.787878787878788 0
0.797979797979798 0
0.808080808080808 0
0.818181818181818 0
0.828282828282828 0
0.838383838383838 0
0.848484848484849 0
0.858585858585859 0
0.868686868686869 0
0.878787878787879 0
0.888888888888889 0
0.898989898989899 0
0.909090909090909 0
0.919191919191919 0
0.929292929292929 0
0.939393939393939 0
0.94949494949495 0
0.95959595959596 0
0.96969696969697 0
0.97979797979798 0
0.98989898989899 0
1 0
};
\addplot [semithick, chocolate, opacity=1.0]
table {%
0 6.66722529143215e-17
0.0101010101010101 0.00445324322208762
0.0202020202020202 0.00890648644417524
0.0303030303030303 0.0133597292006016
0.0404040404040404 0.0178129728883505
0.0505050505050505 0.0222662147134542
0.0606060606060606 0.0267194584012032
0.0707070707070707 0.0311727002263069
0.0808080808080808 0.035625945776701
0.0909090909090909 0.0400791876018047
0.101010101010101 0.0443414002656937
0.111111111111111 0.0468843914568424
0.121212121212121 0.0494273863732815
0.131313131313131 0.0519703775644302
0.141414141414141 0.054513368755579
0.151515151515152 0.0570563636720181
0.161616161616162 0.0595993548631668
0.171717171717172 0.0621423460543156
0.181818181818182 0.0646853372454643
0.191919191919192 0.0672283321619034
0.202020202020202 0.0699705481529236
0.212121212121212 0.0735096335411072
0.222222222222222 0.0770487114787102
0.232323232323232 0.0805877894163132
0.242424242424242 0.0841268673539162
0.252525252525253 0.0876659378409386
0.262626262626263 0.0912050232291222
0.272727272727273 0.0947441011667252
0.282828282828283 0.0982831716537476
0.292929292929293 0.101822257041931
0.303030303030303 0.105297692120075
0.313131313131313 0.108624674379826
0.323232323232323 0.111951656639576
0.333333333333333 0.115278638899326
0.343434343434343 0.118605613708496
0.353535353535354 0.121932603418827
0.363636363636364 0.125259593129158
0.373737373737374 0.128586560487747
0.383838383838384 0.131913542747498
0.393939393939394 0.135240525007248
0.404040404040404 0.137447819113731
0.414141414141414 0.137975573539734
0.424242424242424 0.138503342866898
0.434343434343434 0.139031112194061
0.444444444444444 0.139558881521225
0.454545454545455 0.140086635947227
0.464646464646465 0.140614405274391
0.474747474747475 0.141142174601555
0.484848484848485 0.141669929027557
0.494949494949495 0.142197698354721
0.505050505050505 0.143395394086838
0.515151515151515 0.145263016223907
0.525252525252525 0.147130638360977
0.535353535353535 0.148998245596886
0.545454545454546 0.150865867733955
0.555555555555556 0.152733489871025
0.565656565656566 0.154601097106934
0.575757575757576 0.156468704342842
0.585858585858586 0.158336326479912
0.595959595959596 0.160203948616982
0.606060606060606 0.161124616861343
0.616161616161616 0.161413997411728
0.626262626262626 0.161703363060951
0.636363636363636 0.161992743611336
0.646464646464647 0.16228212416172
0.656565656565657 0.162571504712105
0.666666666666667 0.162860870361328
0.676767676767677 0.163150250911713
0.686868686868687 0.163439631462097
0.696969696969697 0.16372899711132
0.707070707070707 0.161335721611977
0.717171717171717 0.157792672514915
0.727272727272727 0.154249608516693
0.737373737373737 0.150706574320793
0.747474747474748 0.147163525223732
0.757575757575758 0.143620476126671
0.767676767676768 0.140077412128448
0.777777777777778 0.136534363031387
0.787878787878788 0.132991299033165
0.797979797979798 0.129448264837265
0.808080808080808 0.123538792133331
0.818181818181818 0.117037773132324
0.828282828282828 0.110536761581898
0.838383838383838 0.104035750031471
0.848484848484849 0.0975347384810448
0.858585858585859 0.0910337641835213
0.868686868686869 0.0845327526330948
0.878787878787879 0.0780317410826683
0.888888888888889 0.0715307295322418
0.898989898989899 0.0650297179818153
0.909090909090909 0.0585269257426262
0.919191919191919 0.0520239658653736
0.929292929292929 0.0455209650099277
0.939393939393939 0.0390179641544819
0.94949494949495 0.032514963299036
0.95959595959596 0.0260119624435902
0.96969696969697 0.0195089634507895
0.97979797979798 0.0130060007795691
0.98989898989899 0.00650300038978457
1 0
};
\end{axis}

\end{tikzpicture}


==> figures/raw/learned_functions_pspnet/vf_epoch_40000_layer_4.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate}{RGB}{210,105,30}
\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle x\)},
xmin=0, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel style={rotate=-90.0},
ylabel={\(\displaystyle v(x)\)},
ymin=-0.108200061321259, ymax=0.439402747154236,
ytick style={color=black}
]
\addplot [semithick, black, dashed]
table {%
0 0
0.0101010101010101 0
0.0202020202020202 0
0.0303030303030303 0
0.0404040404040404 0
0.0505050505050505 0
0.0606060606060606 0
0.0707070707070707 0
0.0808080808080808 0
0.0909090909090909 0
0.101010101010101 0
0.111111111111111 0
0.121212121212121 0
0.131313131313131 0
0.141414141414141 0
0.151515151515152 0
0.161616161616162 0
0.171717171717172 0
0.181818181818182 0
0.191919191919192 0
0.202020202020202 0
0.212121212121212 0
0.222222222222222 0
0.232323232323232 0
0.242424242424242 0
0.252525252525253 0
0.262626262626263 0
0.272727272727273 0
0.282828282828283 0
0.292929292929293 0
0.303030303030303 0
0.313131313131313 0
0.323232323232323 0
0.333333333333333 0
0.343434343434343 0
0.353535353535354 0
0.363636363636364 0
0.373737373737374 0
0.383838383838384 0
0.393939393939394 0
0.404040404040404 0
0.414141414141414 0
0.424242424242424 0
0.434343434343434 0
0.444444444444444 0
0.454545454545455 0
0.464646464646465 0
0.474747474747475 0
0.484848484848485 0
0.494949494949495 0
0.505050505050505 0
0.515151515151515 0
0.525252525252525 0
0.535353535353535 0
0.545454545454546 0
0.555555555555556 0
0.565656565656566 0
0.575757575757576 0
0.585858585858586 0
0.595959595959596 0
0.606060606060606 0
0.616161616161616 0
0.626262626262626 0
0.636363636363636 0
0.646464646464647 0
0.656565656565657 0
0.666666666666667 0
0.676767676767677 0
0.686868686868687 0
0.696969696969697 0
0.707070707070707 0
0.717171717171717 0
0.727272727272727 0
0.737373737373737 0
0.747474747474748 0
0.757575757575758 0
0.767676767676768 0
0.777777777777778 0
0.787878787878788 0
0.797979797979798 0
0.808080808080808 0
0.818181818181818 0
0.828282828282828 0
0.838383838383838 0
0.848484848484849 0
0.858585858585859 0
0.868686868686869 0
0.878787878787879 0
0.888888888888889 0
0.898989898989899 0
0.909090909090909 0
0.919191919191919 0
0.929292929292929 0
0.939393939393939 0
0.94949494949495 0
0.95959595959596 0
0.96969696969697 0
0.97979797979798 0
0.98989898989899 0
1 0
};
\addplot [semithick, chocolate, opacity=1.0]
table {%
0 3.04444896476216e-16
0.0101010101010101 -0.00847921147942543
0.0202020202020202 -0.0169584229588509
0.0303030303030303 -0.0254376344382763
0.0404040404040404 -0.0339168459177017
0.0505050505050505 -0.0423960536718369
0.0606060606060606 -0.0508752688765526
0.0707070707070707 -0.0593544766306877
0.0808080808080808 -0.0678336918354034
0.0909090909090909 -0.0763128995895386
0.101010101010101 -0.0833090245723724
0.111111111111111 -0.0769573375582695
0.121212121212121 -0.0706056505441666
0.131313131313131 -0.0642539635300636
0.141414141414141 -0.057902280241251
0.151515151515152 -0.0515505895018578
0.161616161616162 -0.0451989062130451
0.171717171717172 -0.0388472229242325
0.181818181818182 -0.0324955321848392
0.191919191919192 -0.0261438470333815
0.202020202020202 -0.0174767877906561
0.212121212121212 0.000451613945188001
0.222222222222222 0.0183799900114536
0.232323232323232 0.0363083630800247
0.242424242424242 0.0542367659509182
0.252525252525253 0.0721651166677475
0.262626262626263 0.0900935158133507
0.272727272727273 0.108021914958954
0.282828282828283 0.125950261950493
0.292929292929293 0.143878668546677
0.303030303030303 0.161057204008102
0.313131313131313 0.17648620903492
0.323232323232323 0.191915258765221
0.333333333333333 0.207344308495522
0.343434343434343 0.222773313522339
0.353535353535354 0.23820236325264
0.363636363636364 0.253631412982941
0.373737373737374 0.269060403108597
0.383838383838384 0.28448948264122
0.393939393939394 0.299918532371521
0.404040404040404 0.313462734222412
0.414141414141414 0.324179857969284
0.424242424242424 0.334897011518478
0.434343434343434 0.345614105463028
0.444444444444444 0.3563312292099
0.454545454545455 0.367048352956772
0.464646464646465 0.377765446901321
0.474747474747475 0.388482570648193
0.484848484848485 0.399199694395065
0.494949494949495 0.409916788339615
0.505050505050505 0.41451171040535
0.515151515151515 0.412984400987625
0.525252525252525 0.411457061767578
0.535353535353535 0.409929722547531
0.545454545454546 0.408402413129807
0.555555555555556 0.40687507390976
0.565656565656566 0.405347764492035
0.575757575757576 0.403820425271988
0.585858585858586 0.402293086051941
0.595959595959596 0.400765776634216
0.606060606060606 0.397253781557083
0.616161616161616 0.392418652772903
0.626262626262626 0.387583553791046
0.636363636363636 0.382748395204544
0.646464646464647 0.377913266420364
0.656565656565657 0.373078137636185
0.666666666666667 0.368243008852005
0.676767676767677 0.363407880067825
0.686868686868687 0.358572781085968
0.696969696969697 0.353737652301788
0.707070707070707 0.346824526786804
0.717171717171717 0.339020669460297
0.727272727272727 0.331216841936111
0.737373737373737 0.323413044214249
0.747474747474748 0.315609186887741
0.757575757575758 0.307805359363556
0.767676767676768 0.300001502037048
0.777777777777778 0.292197674512863
0.787878787878788 0.284393817186356
0.797979797979798 0.276590019464493
0.808080808080808 0.262164622545242
0.818181818181818 0.246083930134773
0.828282828282828 0.230003237724304
0.838383838383838 0.213922545313835
0.848484848484849 0.197841852903366
0.858585858585859 0.181761264801025
0.868686868686869 0.165680572390556
0.878787878787879 0.149599879980087
0.888888888888889 0.133519187569618
0.898989898989899 0.117438495159149
0.909090909090909 0.105300351977348
0.919191919191919 0.093600369989872
0.929292929292929 0.0819003134965897
0.939393939393939 0.0702002570033073
0.94949494949495 0.0585002042353153
0.95959595959596 0.046800147742033
0.96969696969697 0.035100094974041
0.97979797979798 0.0234001092612743
0.98989898989899 0.0117000546306372
1 0
};
\end{axis}

\end{tikzpicture}


==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\RD}{\ensuremath{\RR^D}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}
\newcommand{\WHITE}[1]{{{\color{white}{#1}}}}  

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{ForestGreen}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  
\newcommand{\PURPLE}[1]{{{\color{purple}{#1}}}}  
\newcommand{\SEAGREEN}[1]{{{\color{SeaGreen}{#1}}}}  
\newcommand{\NAVYBLUE}[1]{{{\color{NavyBlue}{#1}}}} 
\newcommand{\ORCHID}[1]{{{\color{Orchid}{#1}}}} 


\newcommand{\gr}[1]{{{\color{gray}{#1}}}}  

\definecolor{brown}{RGB}{165,42,42}
\newcommand{\BROWN}[1]{{{\color{brown}{#1}}}}



\newcommand{\FREIFELD}[1]{\textbf{\MAGENTA{[FREIFELD says: #1]}}}
\newcommand{\IRIT}[1]{\textbf{\BLUE{[IRIT says: #1]}}}
\newcommand{\SHAHAF}[1]{\textbf{\GREEN{[SHAHAF says: #1]}}}
\newcommand{\SHIRA}[1]{\textbf{\PURPLE{[SHIRA says: #1]}}}
% Make your own

\newcommand{\TBD}{\RED{[TBD]}}
\newcommand{\TODO}[1]{\RED{[TODO: #1]}}
\newcommand{\ERAN}[1]{\RED{[ERAN: #1]}}

\newcommand{\REPLACE}[2]{\RED{REPLACE:} \BLUE{#1} \RED{WITH:} \BLUE{#2}}


\newcommand{\SEtwo}{\ensuremath{\mathrm{SE}(2)}}


% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}
\bmdefine\bepsilon{\epsilon}


\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bsigma{\sigma}
\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


 \newcommand{\DP}{\mathrm{DP}}
 \newcommand{\DIR}{\mathrm{Dir}}
 \newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

